HiveNAS: Neural Architecture Search using Artificial Bee Colony Optimization

The traditional Neural Network-development process requires substantial expert knowledge and relies heavily on intuition and trial-and-error. Neural Architecture Search (NAS) frameworks were introduced to robustly search for network topologies, as well as facilitate the automated development of Neural Networks. While some optimization approaches -- such as Genetic Algorithms -- have been extensively explored in the NAS context, other Metaheuristic Optimization algorithms have not yet been investigated. In this study, we evaluate the viability of Artificial Bee Colony optimization for Neural Architecture Search. Our proposed framework, HiveNAS, outperforms existing state-of-the-art Swarm Intelligence-based NAS frameworks in a fraction of the time.

==> tables/ResultsTable.tex <==

\begin{table*}[!htbp]
    \centering
    %\rowcolors{0}{}{gray!10}
    
    \small
    \begin{tabular}{M{2.5cm} M{1.35cm} M{2cm} M{1.75cm} M{1.35cm} M{1.5cm}}
        \toprule
        Model & Search Algorithm & Evaluation Strategy & GPU Usage (days) & Params (millions) & CIFAR10 Error (\%) \\
        \midrule
        
        NASNet (\tiny \cite{zoph_2018}) & RL & LFE & 2,000 & 3.30 & 3.41 \\
        
        MetaQNN (\tiny \cite{baker_2016}) & RL & Full Training & 90 $\pm$ 10 & 11.20 & 6.92 \\
        
        PNAS (\tiny \cite{liu_pnas_2018}) & SMBO & LFE & - & 3.20 & 3.41 \\
        
        NAS (\tiny \cite{zoph_2017}) & RL & Full Training & 22,400 & 37.40 & 3.65 \\
        
        SA-NAS-c (\tiny \cite{mo_2021}) & MO & LFE & 0.1 & 3.20 & 2.53 \\ 
        
        EAS (\tiny \cite{cai_2018}) & RL & Weight Inheritance & 17.5 $\pm$ 7.5 & 23.40 & 4.23 \\
        
        LEMONADE (\tiny \cite{elsken_2018})& EA & Weight Inheritance & 40 $\pm$ 16 & 3.40 & 3.60 \\
        
        Efficient NAS (\tiny \cite{pham_2018}) & RL & OS & 0.45 & 4.60 & 2.89 \\
        
        CARS (\tiny \cite{yang_2020}) & EA & OS & 0.4 & 3.60 & 2.62 \\
        
        PNAS (\tiny \cite{niu_2019}) & MO & Weight Inheritance & 0.2 & 2.44 & 4.62 \\
        
        RandomNAS (\tiny \cite{li_2020}) & RS & OS & 2.7 & 4.30 & 2.85 \\
        
        
        DeepSwarm (\tiny \cite{byla_2019}) & MO & LFE & - & - & 11.31 \\
        
        \midrule
        
        HiveNAS &  & & & 5.30 & 12.64 \\
        
        HiveNAS+Aug &  & & & 6.62 & 9.28 \\
        
        HiveNAS+Cutout &  & &  & 7.12 & 9.84 \\
        
        HiveNAS+ResNet &  & &  & 8.96 & 10.01 \\
        
        HiveNAS+ACT & \multirow{-5}{*}{MO} & \multirow{-5}{*}{LFE} & \multirow{-5}{*}{0.3}  & 8.14 & 8.47 \\
        
        \bottomrule
    \end{tabular}
    \bigskip
    \caption{CIFAR10 Results}
    \label{tab:cifar_res_full}
\end{table*}

